Algorithms as Mechanisms: The Price of Anarchy of Relax-and-Round

Many algorithms that are originally designed without explicitly considering incentive properties are later combined with simple pricing rules and used as mechanisms. The resulting mechanisms are often natural and simple to understand. But how good are these algorithms as mechanisms? Truthful reporting of valuations is typically not a dominant strategy (certainly not with a pay-your-bid, first-price rule, but it is likely not a good strategy even with a critical value, or second-price style rule either). Our goal is to show that a wide class of approximation algorithms yields this way mechanisms with low Price of Anarchy. The seminal result of Lucier and Borodin [SODA 2010] shows that combining a greedy algorithm that is an $\alpha$-approximation algorithm with a pay-your-bid payment rule yields a mechanism whose Price of Anarchy is $O(\alpha)$. In this paper we significantly extend the class of algorithms for which such a result is available by showing that this close connection between approximation ratio on the one hand and Price of Anarchy on the other also holds for the design principle of relaxation and rounding provided that the relaxation is smooth and the rounding is oblivious. We demonstrate the far-reaching consequences of our result by showing its implications for sparse packing integer programs, such as multi-unit auctions and generalized matching, for the maximum traveling salesman problem, for combinatorial auctions, and for single source unsplittable flow problems. In all these problems our approach leads to novel simple, near-optimal mechanisms whose Price of Anarchy either matches or beats the performance guarantees of known mechanisms.

==> half-edges.tex <==
An improved approximation algorithm for max-TSP has been presented by \citet{PaluchEZ12}. The key idea is to compute a cycle cover that does not contain cycles of length $2$. However, computing such a cycle cover would be NP-hard, therefore \citeauthor{PaluchEZ12} relax the constraints further by allowing half-edges. Informally spoken, in a cycle cover without $2$-circles but with half-edges, each vertex still has in- and out-degree exactly $1$. The difference is that the orientation of one edges does not need to be consistent between its two endpoints. That is, the edge can can serve as the ingoing (or outgoing) for both endpoints. However, it is not possible that a single edge serves as both ingoing and outgoing edge for a vertex.

Formally, these constraints can be modeled as follows. A pair of directed edges $(u, v)$ and $(v, u)$ in the original graph is represented by an additional vertex $v_{u, v}$ and directed edges $(u, v_{u, v})$, $(v_{u, v}, v)$, $(v, v_{u, v})$, and $(v_{u, v}, u)$. In a cycle cover without $2$-circles but with half-edges, either none or exactly two of these edges are included and every (original) vertex has indegree and outdegree exactly $1$.

\citeauthor{PaluchEZ12} showed that a cycle cover without $2$-circles but with half-edges can be computed in polynomial time. Furthermore, it is possible to derive three Hamiltonian cycles such that each half-edge is included in at least one of these cycles. Choosing one of these at random, we get an oblivious rounding scheme.

==> symmetric-cas.tex <==
A concrete instantiation of the packing integer program are \emph{combinatorial auctions with symmetric valuations}. 

For symmetric valuations, $\lvert S \rvert = \lvert S' \rvert$ implies $v_i(S) = v_i(S')$ for all $i$. The bids also need to fulfill this assumption. We also write $v_{i,j}$ respectively $b_{i,j}$ to denote the respective values for $\lvert S \rvert = j$.

In this case, there are two canonical relaxations. One based on set variables
\begin{align*}
\max & \sum_{i \in N} \sum_{S \subseteq [m]} b_i(S) \bar{x}_{i, S} \\
\text{s.t.} & \sum_{i \in N} \sum_{S: j \in S} x_{i, S} \leq 1 && \text{ for all $j \in [m]$} \\
& \sum_{S} x_{i, S} \leq 1 && \text{ for all $i \in N$} \\
& x_{i, S} \geq 0 && \text{ for all $i \in N$, $S \subseteq [m]$}
\end{align*}
and one based on cardinality variables
\begin{align*}
\max & \sum_{i \in N} \sum_{k \in [m]} b_{i,k} \bar{x}_{i, k} \\
\text{s.t.} & \sum_{i \in N} \sum_{k \in [m]} k \bar{x}_{i, k} \leq m && \\
& \sum_{k \in [m]} \bar{x}_{i, k} \leq 1 && \text{ for all $i \in N$} \\
& \bar{x}_{i, k} \geq 0 && \text{ for all $i \in N$, $k \in [m]$}
\end{align*}

Fortunately, both relaxations are equivalent: Feasible fractional solutions can be translated without loss and in both cases integral solutions correspond to feasible item allocations of the same value.

From the second relaxation it can be seen that this is a indeed a special case of the LP relaxation of the general integer packing program, in which the matrix $A$ has a single row $(1,\dots,K)$ and $c = m$. Also the parameter $d$ can easily be seen to be equal to $1$.

\subsection{Smoothness}

Since this is a special case of the more general packing integer program problem in which $d = 1$, the above analysis shows that the LP relaxation is $(2,1/2)$-smooth.

\subsection{Fair Rounding}

Instead of invoking the result of \cite{BansalKNS10}, we describe a (simpler) oblivious and fair rounding scheme (with a slightly worse, but still constant fairness guarantee).

Given a fractional allocation of $m$ items, let $\bar{x}_{i, j}$ be the overall fraction that bidder $i$ gets of sets of size at most $j$. Note that by (fractional) feasibility, we have $\sum_{i \in N} \sum_{j \in [m]} j \bar{x}_{i, j} \leq m$.

To round $\bar{x}$, proceeds as follows. Flip a coin.
\begin{itemize}
\item If heads, set $q_{i, j} = \bar{x}_{i, j}$ for all $j \leq \frac{m}{2}$ $q_{i, j} = 0$ for all $j > \frac{m}{2}$.
\item If tails, set $q_{i, j} = 0$ for all $j \leq \frac{m}{2}$ $q_{i, j} = \bar{x}_{i, j}$ for all $j > \frac{m}{2}$.
\end{itemize}
Choose for each bidder $i$ independently at random a value $Q_i$ with $0 \leq Q_i \leq m$, where $\Pr{Q_i = j} = \frac{q_{i, j}}{4}$ and $Q_i = 0$ with the remaining probability. If $\sum_i Q_i \leq m$, set $R_i = Q_i$ for all $i$; otherwise set $R_i = 0$ for all $i$. Use $R_i$ for the allocation.

We now bound the probability that $R_i = Q_i$, conditioned on $Q_i = j$. Observe that if the coin showed heads, we have $j \leq \frac{m}{2}$. Therefore, for $R_i = Q_i$, it suffices to have $\sum_{k \neq i} Q_k \leq \frac{m}{2}$.  If the coin showed tails, all $Q_k$ only take values $0$ or more than $\frac{m}{2}$. For this reason, it also suffices to have $\sum_{k \neq i} Q_k \leq \frac{m}{2}$ for $R_i = Q_i$.

In either case, we have $\Ex{\sum_{k \neq i} Q_k} \leq \sum_{k \neq i} \sum_{j'} j' \frac{\bar{x}_{k, j'}}{4} \leq \frac{m}{4}$, and therefore $\Pr{\sum_{k \neq i} Q_k > \frac{m}{2} \growingmid Q_i = j} \leq \frac{1}{2}$ by Markov's inequality and independence. This gives us $\Pr{R_i = j \growingmid Q_i = j} \geq \frac{1}{2}$.

Overall, we get $\Pr{R_i = j} \geq \frac{\bar{x}_{i, j}}{16}$.

\subsection{Counter Example for Optimal, Integral Solution}\label{sec:symmetric-cas-example}

Consider $m$ items, $m + 2$ bidders. For bidders $i = 1, \ldots, m$, we have $v_i(S) = 1$ for each $S \neq \emptyset$. For bidders $i = m + 1$ and $i = m + 2$, we have $v_i([m]) = 2$ and $v_i(S) = 0$ for $S \neq [m]$. It is a pure Nash equilibrium if $b_i(S) = 0$ for  $i = 1, \ldots, m$ and $b_i = v_i$ for $i = m + 1$ and $i = m + 2$.
